How do humans perceive adversarial text? A reality check on the validity and naturalness of word-based adversarial attacks

Natural Language Processing (NLP) models based on Machine Learning (ML) are susceptible to adversarial attacks -- malicious algorithms that imperceptibly modify input text to force models into making incorrect predictions. However, evaluations of these attacks ignore the property of imperceptibility or study it under limited settings. This entails that adversarial perturbations would not pass any human quality gate and do not represent real threats to human-checked NLP systems. To bypass this limitation and enable proper assessment (and later, improvement) of NLP model robustness, we have surveyed 378 human participants about the perceptibility of text adversarial examples produced by state-of-the-art methods. Our results underline that existing text attacks are impractical in real-world scenarios where humans are involved. This contrasts with previous smaller-scale human studies, which reported overly optimistic conclusions regarding attack success. Through our work, we hope to position human perceptibility as a first-class success criterion for text attacks, and provide guidance for research to build effective attack algorithms and, in turn, design appropriate defence mechanisms.

==> Old_files/RQs_old.tex <==
\section{Research questions}
Our research studies whether textual adversarial examples respects the conditions to be adversarial from the human perspective. 

Initially, we assess the validity requirement, which demands that the adversarial example preserve the same class as the original examples during human inspection. 
\begin{description}
\item[\bf RQ1 (Validity):] \em Do adversarial examples change the class of the text ?
\end{description}
Although adversarial perturbation introduce individual character or word level perturbation, they should not change the semantics of the text. For example, in a sentiment analysis task if the original text is having a negative sentiment for humans, the perturbed text should preserve this meaning and not transform it in a positive sentiment. We evaluate this research question by asking the participants on our survey to label original and adversarial texts according to the task of the dataset(i.e positive or negative sentiment)

Next, we evaluate the concepts related to naturalness of adversarial examples that demands for adversarial examples to be as realistic as possible. 

Initially, we evaluate the suspiciousness level of adversarial examples. 

\begin{description}
\item[\bf RQ2 (Naturality - Suspicioussness):] \em Are the adversarial examples really non-suspicious?
\end{description}
Adversarial examples should look like they are written by humans and not some artificial system. For example, in a text of Early Modern English 
if we find words of Modern English like ``gonna", this would raise suspiciousness  since these words did not exist at that period of time. We answer this question by asking the participants to label original and adversarial examples into ``Written by human" or ``Computer altered" category.  
 
Next, we evaluate if humans are able to detect the actual perturbation. 
\begin{description}
\item[\bf RQ3 (Naturality - Detectability):] \em Do humans base their suspiciousness judgment on the adversarial perturbations that caused misclassification? 
\end{description}
The suspicion that a text seems computer-altered might come from different sources of typos, meaning fluctuations etc. In order to evaluate if humans can point to the actual perturbations, we ask them to select the words they believe are computer altered in case they think the text was altered. 



\begin{description}
\item[\bf RQ4 (Naturality - Gramaticality):]\hfill \\
\em a) Do adversarial examples respect the grammaticality according to the human participants? \hfill \\
 b) Do adversarial examples introduce grammar errors?  
\end{description}


Lastly, to ensure that the adversarial examples are as natural as possible, we evaluate their meaning. 
\begin{description}
\item[\bf RQ5 (Naturality - Meaning):] \hfill \\
\em a) Are adversarial examples meaningful for human participants? \hfill \\
b) Do adversarial examples preserve the meaning of the original sentences?
\end{description}
For the first sub-question we ask the participants to label adversarial sentences as ``Not clear at all", ``Barely clear", ``Clear" and ``Very clear". For the second sub-question we present both the original and adversarial sentence and ask the participants to answer if the meaning is preserved from the first text to the second with ``No, not at all", ``Somehow", ``Almost", ``Yes, absolutely". 


Lastly, we pose the question about the current attacks and their performance related to the above criteria of validity and naturality. 
\begin{description}
\item[\bf RQ6 ():] \hfill \\
\em What is the status of the existing attacks regarding validity and naturality? \hfill
\end{description}
There already exists over 20 textual adversarial attacks and new ones are still being published. We investigate if the existing attacks have already reached a mature state where they have a high validity and naturalness when evaluated by human participants, or if improvements are to be made in the future research and which areas. 


==> Old_files/Results_old.tex <==
\section{Analysis and Results}
\subsection{Validity}
In this section we analyse whether adversarial text preserves the original sentiment, hence remaining valid as described in Section 2.2. We calculate the accuracy of the human participants on labelling the sentiment of original and adversarial text, considering the labels provided originally with the dataset as the ground truth. We use proportions tests to test for statisitcal significance. 

Firstly, we analyze the overall data. The results show that  human annonators were 88.78\%  accurate for original text and 71.86\% for adversarial text when giving a sentiment label. From a left-tailed two sampled proportions test we obtain a critical value of $Z=-12.79<=-2.33$ and $p=9.92e^{-38}<= 0.01$. This demonstrates that the labeling accuracy of humans is statistically lower for adversarial texts, which means they are not always valid. 

Next we analyse the results for individual attacks, to understand if there is a difference in the validity of adversarial examples they generate. From the results given in Table \ref{table:rq1_attack}, we observe that for some attacks the labelling accuracy is over 80\%,  similar to original text. However, for attacks like BAE and CLARE the sentiment labelling accuracy is very close to random, between 50\% and 60\%. These attacks perform poorly in preserving the original sentiment of text, therefore they would be ineffective at their adversarial goal.


\begin{table}[ht!]
\begin{tabular}{@{}ll@{}}
\toprule
Attack            & Accuracy \\ \midrule
$^{a}$BAE      & 55.4$^{b,d,e,f,h,i}$    \\
$^{b}$BERTAttack  & 71.1$^{a,c,e,f,i}$     \\
$^{c}$CLARE         & 55.4$^{b,d,e,f,h,i}$    \\
$^{d}$FGA        & 84.2$^{a,c,g}$     \\
$^{e}$IGA      & 87.5$^{a,b,c,g}$     \\
$^{f}$Kuleshov      & 86.8$^{a,b,c,g,h}$     \\
$^{g}$PSO       & 63.5$^{d,e,f,h,i}$       \\
$^{h}$PWWS       & 74.8$^{a,c,f,g,i}$     \\
$^{i}$TextFooler & 85.9$^{a,b,c,g,h}$     \\ \bottomrule
\end{tabular}
\caption{Sentiment labelling accuracy for adversarial text according to the attack method. Superscripts indicate statistical difference observed with proportion tests ($\alpha=0.01$). 
\label{table:rq1_attack}}
\end{table}

We now study the effect that the perturbation size has on the sentiment labelling accuracy. Figure \ref{fig:rq1_perturbation_size} shows for each perturbation size, the average success rate between attacks  as well as the minimum and maximum accuracy reached by the attacks.  A Pearson correlation test of $r$=-0.031 (99\% CI = [-0.033, -0.029], p=0.85 $>0.01$) confirmed the visual observation that there is no linear correlation between the perturbation size and the sentiment labelling accuracy. Additionally, we ran Pearson correlation tests for individual attacks, and we could not find strong correlation above 0.5 or below -0.5 for any of them.  The graph also shows that there is a considerable gap between the attack with the lowest accuracy and the highest accuracy, for some percentages  even higher than 40\%. 

\begin{figure}[ht!]
\includegraphics[width=\linewidth]{figures/rq1_shaded.JPG}
\caption{Effect of perturbation size on sentiment labelling accuracy.}
\label{fig:rq1_perturbation_size}
\end{figure}

Lastly, we study whether the participants' English language proficiency has any effect on their sentiment labelling accuracy. The results in Table \ref{table:rq1_language} show that for original text, participants with higher proficiency are more accurate. However, the only statistical difference  with the proportions test is observed between limited working proficiency and native/bilingual. For adversarial text, the sentiment labelling accuracy is not impacted by language proficiency. 

\begin{table}[ht!]
\begin{tabular}{@{}lll@{}}
\toprule
Language proficiency        & Original & Adversarial \\ \midrule
$^{a}$Limited working & 84.4$^{c}$     & 72.4        \\
$^{b}$Professional    & 88.5      & 72.6        \\
$^{c}$Native/Bilingual            & 91.0$^{a}$     & 70.7        \\ \bottomrule
\end{tabular}
\caption{Sentiment labelling accuracy by language proficiency. Superscripts indicate statistical difference observed with proportion tests ($\alpha=0.01$)}
\label{table:rq1_language}
\end{table}

\noindent\fbox{%
    \parbox{\columnwidth}{%
Adversarial examples are not always valid, although there exist a difference between the attacks. Some of the attacks render almost 50\% of their output as invalid, while others keep the same validity levels as for original text. The perturbation level and the language proficiency of the participant do not impact the validity results for adversarial text. 
    }%
}

\subsection{Naturality - Suspicion}

We investigate whether adversarial texts raise the suspicion of human evaluators. For that purpose, we analyze the accuracy of human participants on labeling text as "Computer-altered" or "Written by humans". 

The results show that humans annotators are statistically better at identifying the original text than the adversarial text - 78.57\% versus 60.33\% (left-tailed two-sampled proportion test of $Z=-11.83<=-2.33$ and $p=1.30e^{-32}<= 0.01$). However, 60.33\% of the adversarial examples cannot bypass a human check. 


% This is a much higher percentage than previously reported. 
% The human annotators were 78.57\% successful in labelling original text as human written and 60.33\% successful in labelling adversarial text as computer-altered. We conduct a  left-tailed two sampled proportions test and obtain $Z=-11.83<=-2.33$ and $p=1.30e^{-32}<= \alpha=0.01$. This demonstrates that the accuracy of identifying computer-altered text is statistically lower than the accuracy of identifying human written text.
% The adversarial attacks introduce perturbation that raises the suspicion level. Only 39.77\% of them manage to go uncovered, \textcolor{red}{which is a much higher percentage than what was reported in previous studies.}   These results show that adversarial texts generated with existing attacks clearly do not  respect suspicion constraint, contrary to what is assumed. 


To understand whether different attacks produce examples that raise different level of suspicion, we analyze the data separately for each attack and present the results in Table \ref{table:rq2_attack}. The attack that produced the less suspicious examples is FGA, where participants labelled 46.55\% of the text as adversarial. However, this still remains a high value, considering that participants labelled only 21.43\% of the original texts as adversarial. Other attacks produce more suspicious examples, 5 of them having adversarial examples detected more than 60\% of the time.

\begin{table}[ht!]
\begin{tabular}{@{}ll@{}}
\toprule
Attack            & Accuracy \\ \midrule
$^{a}$BAE      & 50.6 $^{b,f,g,h}$   \\
$^{b}$BERTAttack  & 63.9 $^{a,d}$    \\
$^{c}$CLARE         & 55.9 $^{g}$     \\
$^{d}$FGA        & 46.5 $^{b,f,g,h}$    \\
$^{e}$IGA      & 59.1      \\
$^{f}$Kuleshov      & 63.9 $^{a,d}$     \\
$^{g}$PSO       & 68.5 $^{a,c,d}$      \\
$^{h}$PWWS       & 65.5 $^{a,d}$    \\
$^{i}$TextFooler & 61.5     \\ \bottomrule
\end{tabular}
\caption{Accuracy of labelling adversarial text as computer-altered based on the attack. Superscripts indicate statistical difference observed with proportion tests ($\alpha=0.01$). 
\label{table:rq2_attack}}
\end{table}

Next, we analyze the effect that the perturbation size of adversarial examples has on human suspicion.  The positive linear correlation observed visually in Figure \ref{fig:rq1_perturbation_size} was confirmed with a Pearson correlation test of $r=0.72$ (99\% CI = [0.71, 0.72], p=3.18$e^{-7} <= 0.01$). Introducing higher perturbation levels in adversarial text, will increase the suspicion levels of humans. For individual attacks, we found that only for BERTAttack exists a significant positive correlation ($r=0.50$, p=0.0014$e^{-7} < 0.01$). For the rest of the attacks the correlation coefficient was between 0 and 0.50  and $p>0.01$, resulting in statistically insignificant findings.

\begin{figure}[ht!]
\includegraphics[width=\linewidth]{figures/rq2_shaded.JPG}
\caption{Effect of perturbation size on labelling adversarial text as computer-altered.}
\label{fig:rq2_perturbation_size}
\end{figure}


Finally, we analyze the effect that participants' language proficiency has on the suspicion results. Table \ref{table:rq2_language} shows that  for original examples, participants with professional proficiency are more suspicious and label the original text more often as computer-altered compared to limited working proficiency and native/bilinguals. The same behaviour is observed for adversarial examples, people with professional proficiency are more suspicious, hence achieving a higher accuracy compared to the other two levels of proficiency. 

\begin{table}[ht!]
\begin{tabular}{@{}lll@{}}
\toprule
Language proficiency        & Original & Adversarial \\ \midrule
$^{a}$Limited working & 79.3     & 54.8 $^{b}$       \\
$^{b}$Professional    & 74.2 $^{c}$     & 64.6 $^{a,c}$        \\
$^{c}$Native/Bilingual            & 84.1 $^{b}$     & 57.0 $^{b}$       \\ \bottomrule
\end{tabular}
\caption{Accuracy of labelling adversarial text as computer-altered based on language proficiency. The superscripts indicate the statistical difference observed with proportion tests ($\alpha=0.01$)}
\label{table:rq2_language}
\end{table}

\noindent\fbox{%
    \parbox{\columnwidth}{%
Adversarial examples are suspicious to human participants on 60.3\% of the times. Only one attack produces examples that are suspicious, less than 50\% of the times. Higher perturbation rates result in up to \textcolor{red}{XXX\%} increase of suspicion levels. People with professional English proficiency are more suspicious and tend to label text more often as computer-altered. 
    }%
}

\subsection{Naturality - Detectability}
As part of the naturality evaluation, we study whether humans can detect  the words that were perturbed by adversarial attacks. We compute the detection rate as the percentage of perturbed words that are correctly guessed by the participants. \textcolor{red}{In Appendix ZZZ you will find the results for the inverse ratio, the percentage of the guessed words that are actually perturbed.} We study this question in two scenarios, when the participants can select an unlimited number of suspicious fords or a fixed number. 

The results showed that when the number of choices is limited, humans detect perturbed words at a higher rate; on average, 27.54\% of perturbed words were detected for unlimited choices and 52.38\% for a fixed number (Mann-Whitney U Test of $Z=-288.34 <= -2.576$ and $p=1.32e-79= 0.01$). A possible explanation can be that humans underestimate the number of perturbed words. When faced with an unlimited number of choices, they choose the few that are more obvious. This reduces the time of their analysis and their mental burden. When participants are required to select a fixed number of words, they are forced to choose beyond the most obvious perturbations. Even if they choose the least obvious words randomly to reduce their mental burden, the detection rate can increase by chance.

As with the other criteria for naturality, we analyze the detectability rates according to the attack in Table \ref{table:rq3_attack}. Similar to the general trend, the detection rate increases if participants are limited in their number of choices for all nine attacks. Furthermore, for unlimited choices, there  is a significant difference of 18.6\% between the lowest (BAE 18.2\%) and  highest detection rate (Kuleshov 36.8\%). For a fixed number of choices, the difference between the lowest (Clare 39.4\%) and the highest(Kuleshov 65.9\%) detection rate slightly increases to 26.5\%. Kuleshov attack that has the highest detection rate, was one of top three attacks in terms of suspicion for humans. 

\begin{table}[ht!]
\begin{tabular}{@{}lll@{}}
\toprule
Attack                  & Unlimited & Exact \\ \midrule
$^{a}$BAE      & 18.2$^{e,f,g,h,i}$              & 45.3$^{e,f,g,h,i}$         \\
$^{b}$BERTAttack  & 19.5$^{f,g,h}$             & 44.3$^{e,f,g,h,i}$         \\
$^{c}$CLARE         & 25.4$^{f,g,h}$             & 39.4$^{e,f,g,h,i}$         \\
$^{d}$FGA        & 23.1$^{f,g,h}$            & 46.3$^{f,h}$           \\
$^{e}$IGA      & 31.4$^{a}$             & 57.8  $^{a, b, c}$        \\
$^{f}$Kuleshov      & 36.8$^{a, b, c, d}$             & 65.9 $^{a, b, c, d, g, i}$           \\
$^{g}$PSO       & 32.2$^{a, b, c, d}$              & 54.7 $^{a, b, c, f, h}$         \\
$^{h}$PWWS       & 33.3$^{a, b, c, d}$              & 63.7$^{a, b, c, d, g, i}$            \\
$^{i}$TextFooler & 27.8$^{a}$              & 54.7$^{a, b, c, f, h}$          \\ \bottomrule
\end{tabular}
\caption{Detectability of perturbed words based on the attack. Superscripts indicate statistical difference observed with Mann Whitney U Test ($\alpha=0.01$). 
\label{table:rq3_attack}}
\end{table}


We study the effect that the perturbation size has on detection rate. Figure \ref{fig:rq3_perturbation_size} show that there is no linear relation for unlimited word choices between the perturbation size and detection rate, confirmed with a Pearson correlation test of $r$=0.026 (99\% CI = [0.025, 0.026], p=0.30 $>0.01$). We did not observe strong linear relationship of  above 0.5 or below -0.5 for individual attacks either. 

In the scenario when the participants have to choose exact number of word, no strong linear relation was observed  between the perturbation size and detection rate, confirmed by a Pearson correlation test of $r$=-0.007 (99\% CI = [-0.0074, -0.0067], p=0.80 $>0.01$). For individual attacks, there was no strong linear correlation of above 0.5 or below -0.5. 

\begin{figure}[ht!]
\includegraphics[width=\linewidth]{figures/rq3_shaded.JPG}
\caption{Effect of perturbation size on detection rate.}
\label{fig:rq3_perturbation_size}
\end{figure}


Finally, we study the effect of language proficiency of participants on their detection rates.  Table \ref{table:rq3_language}.  For all three language proficiencies, the detection rate increases from unlimited to fixed number of choices scenario. Although, for both scenarios, there were no statistical differences on the reported detection rates by different language proficiencies groups.

\begin{table}[ht!]
\begin{tabular}{lll}
\hline
Language proficiency              & Unlimited & Exact \\ \hline
$^{a}$Limited working proficiency & 23.5      & 48.6    \\
$^{b}$Professional proficiency    & 28.6      & 52.5    \\
$^{c}$Native/Bilingual            & 27.9      & 53.8    \\ \hline
\end{tabular}
\caption{Detection rate based on language proficiency. Superscripts indicate statistical difference observed with Mann Whitney U Test($\alpha=0.01$)}
\label{table:rq3_language}
\end{table}

\noindent\fbox{%
    \parbox{\columnwidth}{% 
    Humans can detect up to 27.54\% of perturbed words when they are not limited on their word choices, and up to 52.38\% when restricted to a fixed number of words. The detection rate between attacks varies up to 26.5\%. The perturbation size and participants' language efficiency does not have an effect on the detection rate. 
    }%
}

\subsection{Naturality - Grammaticality}

In this section, we study whether adversarial examples respect grammar rules according to the human participants and whether the adversarial perturbations introduce new errors. To understand the extent to which the human judgment is "realistic", we analyse the grammar error rates reported by LanguageTool grammar checker.

The results show that humans report higher rate of present grammar error compared to LanguageTools, respectively 66.9\% vs 53.3\% for original texts and 38.9\% vs 17.7\% for adversarial text. Additionally, even though the option "Not sure" was present, the participants have selected it only 12.6\% of the time for original text and 17.1\% of the times for adversarial text. This shows that they are confident that they can identify the presence of grammar errors. 

Similarly, the rate of introduced grammar errors by the adversarial perturbations for humans(40.6\%) is higher than for LanguageTool(17.7\%). 


% The result in Table \ref{table:rq4_general} show that humans  We observe that humans are always reporting grammar errors at a much higher scale than LanguageTools. \textcolor{red}{Add explanation why it happens}. Additionally, even though the option "Not sure" was present they decided to use only less than 20\% of times, which shows that they are confident that they can make a choice even though if we would consider LanguageTools as our groundtruth their error rate is as high as 28.2\%. 

% \begin{table}[ht!]
% \small
% \begin{tabular}{@{}lllll@{}}
% \cmidrule(l){2-5}
%                                 &             & Yes          & No          & Not  \\
%                                 &             &              &             & sure \\ \midrule
% \multicolumn{1}{l|}{Errors}     & Original    & 66.9 (53.3) & 20.5(46.7) & 12.6 \\
% \multicolumn{1}{l|}{present}    & Adv. & 38.9 (17.7) & 44.0(82.3) & 17.1 \\ \midrule
% \multicolumn{1}{l|}{Errors}     & Adv. & 40.6 (12.4) & 46.4(87.6) & 13.0 \\
% \multicolumn{1}{l|}{added} &             &              &             &      \\ \bottomrule
% \end{tabular}
% \caption{Percentage of grammar errors detected by human evaluators. The numbers in bracket represent the errors found automatically with LanguageTools grammar checker. } 
% \label{table:rq4_general}
% \end{table}

The results for individual attacks are shown in Table \ref{table:rq4_attack}. When judging if the texts contain grammar errors, humans report the highest rates (over 40\%) for CLARE, BAEgarg2019, FGA. However, this does not correspond to the output of LanguageTools given in brackets. LanguageTools ranks CLARE in the top three attacks with the least errors. The difference between the lowest and the highest rate in this case is of 30.3\%. 

Similarly to the above results, when judging if the adversarial examples introduced errors the top reported attacks by humans do not always match the ranking of LanguageTool. The difference on added errors by attack varies up to 39\%. 

\begin{table}[]
\begin{tabular}{@{}lll@{}}
\toprule
Attack     & Errors present & Errors added \\ \midrule
BAE        & 44.2 (3.4)     & 29.0 (2.8)      \\
BERTAttack & 23.7 (22.7)    & 55.4 (12.0)    \\
CLARE      & 53.8 (9.2)     & 16.4 (2.2)   \\
FGA        & 44.6 (22.8)    & 34.5 (10.3)  \\
IGA        & 36.4 (22.7)    & 47.0 (16.7)    \\
Kuleshov   & 37.6 (16.6)    & 43.9 (12.1)  \\
PSO        & 37.4 (8.6)     & 39.1 (7.1)   \\
PWWS       & 34.5 (27.0)    & 48.0 (18.4)    \\
TextFooler & 39.1 (34.4)    & 50.5 (29.6)   \\ \bottomrule
\end{tabular}
\caption{Percentage of texts that contain and introduced grammar errors by attack as reported by human evaluators.  The numbers in brackets represent the results obtained with LanguageTools grammar checker. } 
\label{table:rq4_attack}
\end{table}


% \begin{table*}[ht!]
% \begin{tabular}{@{}llll|lll@{}}
% \cmidrule(l){2-7}
%                         & \multicolumn{3}{l|}{Error present}     & \multicolumn{3}{l}{Error added}        \\ \midrule
% Attack                  & Yes          & No           & Not sure & Yes          & No           & Not sure \\ \midrule
% $^{a}$BAE      & 44.2 (3.4)  & 39.9 (96.6) & 15.9     & 29(2.8)     & 61.4 (97.2) & 9.7      \\
% $^{b}$BERTAttack  & 23.7 (22.7) & 59.8 (77.3) & 16.5     & 55.4 (12)   & 32.1 (88)   & 12.5     \\
% $^{c}$CLARE         & 53.8 (9.2)  & 29.7 (90.8) & 16.4     & 16.4 (2.2)  & 72.7(97.8)   & 10.9     \\
% $^{d}$FGA        & 44.6 (22.8) & 34.7 (77.2) & 20.8     & 34.5 (10.3) & 44.8(89.7)   & 20.7     \\
% $^{e}$IGA      & 36.4 (22.7) & 48.9 (77.3) & 14.8     & 47 (16.7)   & 47(83.3)     & 6.1      \\
% $^{f}$Kuleshov      & 37.6 (16.6) & 45.4 (83.4) & 17.1     & 43.9 (12.1) & 41.6(87.9)   & 14.5     \\
% $^{g}$PSO       & 37.4 (8.6)  & 42.3 (91.4) & 20.3     & 39.1 (7.1)  & 44.2(92.9)   & 16.7     \\
% $^{h}$PWWS       & 34.5 (27)   & 49.6 (73)   & 15.9     & 48 (18.4)   & 39.5(81.6)   & 12.5     \\
% $^{i}$TextFooler & 39.1 (34.4) & 44.3 (65.6) & 16.7     & 50.5(29.6)  & 34.9(70.4)   & 14.5     \\ \bottomrule
% \end{tabular}
% \caption{Percentage of grammar errors detected by human evaluators, split by attack. The numbers in brackets represent the errors found automatically with LanguageTools grammar checker. } 
% \label{table:rq4_attack}
% \end{table*}

Lastly, we study the effect that language proficiency has on our results.  Table \ref{table:rq4_language} shows  the language proficiency does not  have an effect on the errors reported for adversarial examples.  However, it affects the reported rate of errors introduced by adversarial examples on original text. More proficient participants report more added errors, with Native/bilinguals reporting up to 13.3\% more added errors. 

\begin{table}[ht!]
\begin{tabular}{@{}lll@{}}
\toprule
Language proficiency & Errors     & Errors     \\
                     & present    & added      \\ \midrule
Limited working      & 38.8(17.6) & 31.7(12.4) \\
Professional         & 38.3(18)   & 40.1(13.1) \\
Native/bilingual     & 39.7(17.3) & 45.0(11.6)  
\end{tabular}
\caption{Percentage of grammar errors detected by human evaluators  according to their language proficiency. The numbers in brackets represent the errors found automatically with LanguageTools grammar checker. }
\label{table:rq4_language}
\end{table}


\noindent\fbox{%
    \parbox{\columnwidth}{% 
    Humans report both high rate of errors present in adversarial sentences (up to 53.8\% for attack) and added errors by adversarial perturbation (up to 55.4\% per attack). These rates are much higher than what reported by automatic grammar checkers like LanguageTool. The language proficiency of the participants only affected the reported added error rate, not the errors present rate. 
    }%
}


% \begin{table*}[ht!]
% \begin{tabular}{@{}llll|lll@{}}
% \cmidrule(l){2-7}
%                                    & \multicolumn{3}{l|}{Error present} & \multicolumn{3}{l}{Error added}    \\ \midrule
% Language proficiency               & Yes        & No         & Not sure & Yes        & No         & Not sure \\ \midrule
% $^{a}$ Limited working proficiency & 38.8(17.6) & 37.6(82.4) & 23.6     & 31.7(12.4) & 45(87.6)   & 23.3     \\
% $^{b}$ Professional proficiency    & 38.3(18)   & 45.4(82)   & 16.3     & 40.1(13.1) & 45.9(86.9) & 14.1     \\
% $^{c}$ Native/Bilingual            & 39.7(17.3) & 44.8(82.7) & 15.5     & 45(11.6)   & 47.5(88.4) & 7.5     
% \end{tabular}
% \caption{Percentage of grammar errors detected by human evaluators  according to their language proficiency. The numbers in brackets represent the errors found automatically with LanguageTools grammar checker. }
% \label{table:rq4_language}
% \end{table*}

\subsection{Naturality - Meaning}
As a last aspect of naturality, we study whether adversarial texts are meaningful and whether they preserve the meaning of the original texts where they were derived from. To answer these questions, we report the average Likert scores on a scale from 1 to 4 as introduced in Section 2.2. 

% We have averaged the ratings received from the participants on a Likert-item scale of 1 to 4. When presented with only the adversarial examples a rating of 1 means the text meaning is not clear at all and a rating of 4 means the meaning is very clear. When presented with both original and adversarial text, a rating of 1 means that the adversarial text does not preserve the meaning of the original text and a rating of 4 means that adversarial text totally preserves the meaning. 

Results show that humans statistically find the original texts with an average rating of 3.44 more meaningful than adversarial text with an average rating of 2.60 (Mann Whitney U Test of $Z=-412.10 <= - 2.576$ and $p=1.43e^{-142}<=0.01$). Additionally, humans believe that adversarial examples preserve the meaning of the original text only partially. They rate adversarial examples with an average score of 2.11 for their meaning preservation capabilities. As a reminder, a score of 2 corresponds to the option "Somehow" and a score of 3 to "Almost". 


The results for individual attacks are given in Table \ref{table:rq5_attack}. Most of the attacks lay between a score of 2 and 3 regarding the clarity of the meaning. FGA(2.88) and CLARE(3.06) attacks perform the best with scores that indicate almost clear meaning. The meaning preservation capability of the attacks ranges in lower values from 1.7 to 2.67. This last score is reached by FGA, which indicates a core between somehow and almost preserved meaning. 

\begin{table}[ht!]
\begin{tabular}{lll}
\hline
Attack                  & Meaningful & Preserved \\ \hline
$^{a}$BAE      & 2.64$^{d,g,h}$       & 1.7      $^{b, d, e, f, g, h, i}$          \\
$^{b}$BERTAttack  & 2.4 $^{c, d, f, i}$        & 2.07   $^{a,c,d,e,i}$           \\
$^{c}$CLARE         & 2.88 $^{b, g, h}$      & 1.7 $^{b, d, e, f, g, h, i}$     \\
$^{d}$FGA        & 3.06 $^{a, b, e, f, g, h, i}$    & 2.67$^{a,b, c, g, h}$\\
$^{e}$IGA      & 2.7  $^{d, g, h}$      & 2.58  $^{a,b, c, g, h}$             \\
$^{f}$Kuleshov      & 2.71 $^{b, d, g, h}$       & 2.29  $^{a,c, g}$            \\
$^{g}$PSO       & 2.34  $^{a, c, d, e, f, i}$     & 1.99 $^{a,c, d,e, f,i}$              \\
$^{h}$PWWS       & 2.26  $^{a, c, d, e, f, i}$      & 2.09  $^{a,c, d,e,i}$             \\
$^{i}$TextFooler & 2.72    $^{b, d, g, h}$    & 2.47   $^{a,b, c, g, h}$            \\ \hline
\end{tabular}
\caption{Clarity of the meaning and its preservation based on the attack. Superscripts indicate statistical difference observed with Mann Whitney U Test ($\alpha=0.01$). 
\label{table:rq5_attack}}
\end{table}

Next, we study the effect of the perturbation size on clarity of meaning and meaning preservation.  The visualization in Figure \ref{fig:rq5_perturbation_size} shows a slightly negative relationship between the perturbation size and clarity of meaning, which is confirmed by a Pearson correlation test of $r=-0.21$ (99\% CI = [-0.21, -0.21], p=1.17$e^{-17} <= 0.01$). Similarly, we observe a slightly negative relationship even between the perturbation size and the meaning preservation capability, confirmed by a Pearson correlation test of $r=-0.19$ (99\% CI = [-0.19, -0.19], p=1.91$e^{-12} <= 0.01$)

\begin{figure}[ht!]
\includegraphics[width=\linewidth]{figures/rq5_shaded.JPG}
\caption{Effect of perturbation size on meaning and its preservation.}
\label{fig:rq5_perturbation_size}
\caption{Effect of perturbation size on meaning clarity and its preservation.  }
\end{figure}


Finally, we investigate the influence of language proficiency in our results. According to the data in Table \ref{table:rq5_language},  the proficiency level does not statistically affect the clarity of the meaning. Regarding meaning preservation, the group with limited working proficiency assigns a statistically higher score than the native/bilingual group. 

\begin{table}[ht!]
\begin{tabular}{lll}
\hline
Language proficiency              & Meaning & Preservation \\ \hline
$^{a}$Limited working  & 2.65  & 2.26 $^{c}$ \\
$^{b}$Professional     & 2.63  & 2     \\
$^{c}$Native/Bilingual            & 2.55  & 2.15 $^{a}$ \\ \hline
\end{tabular}
\caption{Clarity of the meaning and meaning preservation based on language proficiency. Superscripts indicate statistical difference observed with Mann Whitney U Test($\alpha=0.01$)}
\label{table:rq5_language}
\end{table}

\noindent\fbox{%
    \parbox{\columnwidth}{% 
  Humans find that adversarial text is less meaningful than original text. They as well report that adversarial text somehow preserves the meaning of the original text, but not completely. Higher adversarial perturbation size, renders the text less meaningful and reduces its meaning preserving capabilities. The language proficiency does not have a strong effect on the results reported by humans. 
    }%
}

==> Old_files/results_RQ3_old.tex <==
\textbf{Validity}

We now study the effect that the perturbation size has on the sentiment labelling accuracy. Figure \ref{fig:rq1_perturbation_size} shows for each perturbation size, the average success rate between attacks  as well as the minimum and maximum accuracy reached by the attacks.  A Pearson correlation test of $r$=-0.031 (99\% CI = [-0.033, -0.029], p=0.85 $>0.01$) confirmed the visual observation that there is no linear correlation between the perturbation size and the sentiment labelling accuracy. Additionally, we ran Pearson correlation tests for individual attacks, and we could not find strong correlation above 0.5 or below -0.5 for any of them.  The graph also shows that there is a considerable gap between the attack with the lowest accuracy and the highest accuracy, for some percentages  even higher than 40\%. 

\begin{figure}[ht!]
\includegraphics[width=\linewidth]{figures/rq1_shaded.JPG}
\caption{Effect of perturbation size on sentiment labelling accuracy.}
\label{fig:rq1_perturbation_size}
\end{figure}

Lastly, we study whether the participants' English language proficiency has any effect on their sentiment labelling accuracy. The results in Table \ref{table:rq1_language} show that for original text, participants with higher proficiency are more accurate. However, the only statistical difference  with the proportions test is observed between limited working proficiency and native/bilingual. For adversarial text, the sentiment labelling accuracy is not impacted by language proficiency. 

\begin{table}[ht!]
\begin{tabular}{@{}lll@{}}
\toprule
Language proficiency        & Original & Adversarial \\ \midrule
$^{a}$Limited working & 84.4$^{c}$     & 72.4        \\
$^{b}$Professional    & 88.5      & 72.6        \\
$^{c}$Native/Bilingual            & 91.0$^{a}$     & 70.7        \\ \bottomrule
\end{tabular}
\caption{Sentiment labelling accuracy by language proficiency. Superscripts indicate statistical difference observed with proportion tests ($\alpha=0.01$)}
\label{table:rq1_language}
\end{table}


\textbf{Suspicion}

Next, we analyze the effect that the perturbation size of adversarial examples has on human suspicion.  The positive linear correlation observed visually in Figure \ref{fig:rq1_perturbation_size} was confirmed with a Pearson correlation test of $r=0.72$ (99\% CI = [0.71, 0.72], p=3.18$e^{-7} <= 0.01$). Introducing higher perturbation levels in adversarial text, will increase the suspicion levels of humans. For individual attacks, we found that only for BERTAttack exists a significant positive correlation ($r=0.50$, p=0.0014$e^{-7} < 0.01$). For the rest of the attacks the correlation coefficient was between 0 and 0.50  and $p>0.01$, resulting in statistically insignificant findings.

\begin{figure}[ht!]
\includegraphics[width=\linewidth]{figures/rq2_shaded.JPG}
\caption{Effect of perturbation size on labelling adversarial text as computer-altered.}
\label{fig:rq2_perturbation_size}
\end{figure}


Finally, we analyze the effect that participants' language proficiency has on the suspicion results. Table \ref{table:rq2_language} shows that  for original examples, participants with professional proficiency are more suspicious and label the original text more often as computer-altered compared to limited working proficiency and native/bilinguals. The same behaviour is observed for adversarial examples, people with professional proficiency are more suspicious, hence achieving a higher accuracy compared to the other two levels of proficiency. 

\begin{table}[ht!]
\begin{tabular}{@{}lll@{}}
\toprule
Language proficiency        & Original & Adversarial \\ \midrule
$^{a}$Limited working & 79.3     & 54.8 $^{b}$       \\
$^{b}$Professional    & 74.2 $^{c}$     & 64.6 $^{a,c}$        \\
$^{c}$Native/Bilingual            & 84.1 $^{b}$     & 57.0 $^{b}$       \\ \bottomrule
\end{tabular}
\caption{Accuracy of labelling adversarial text as computer-altered based on language proficiency. The superscripts indicate the statistical difference observed with proportion tests ($\alpha=0.01$)}
\label{table:rq2_language}
\end{table}



\textbf{Detectability}
We study the effect that the perturbation size has on detection rate. Figure \ref{fig:rq3_perturbation_size} show that there is no linear relation for unlimited word choices between the perturbation size and detection rate, confirmed with a Pearson correlation test of $r$=0.026 (99\% CI = [0.025, 0.026], p=0.30 $>0.01$). We did not observe strong linear relationship of  above 0.5 or below -0.5 for individual attacks either. 

In the scenario when the participants have to choose exact number of word, no strong linear relation was observed  between the perturbation size and detection rate, confirmed by a Pearson correlation test of $r$=-0.007 (99\% CI = [-0.0074, -0.0067], p=0.80 $>0.01$). For individual attacks, there was no strong linear correlation of above 0.5 or below -0.5. 

\begin{figure}[ht!]
\includegraphics[width=\linewidth]{figures/rq3_shaded.JPG}
\caption{Effect of perturbation size on detection rate.}
\label{fig:rq3_perturbation_size}
\end{figure}


Finally, we study the effect of language proficiency of participants on their detection rates.  Table \ref{table:rq3_language}.  For all three language proficiencies, the detection rate increases from unlimited to fixed number of choices scenario. Although, for both scenarios, there were no statistical differences on the reported detection rates by different language proficiencies groups.

\begin{table}[ht!]
\begin{tabular}{lll}
\hline
Language proficiency              & Unlimited & Exact \\ \hline
$^{a}$Limited working proficiency & 23.5      & 48.6    \\
$^{b}$Professional proficiency    & 28.6      & 52.5    \\
$^{c}$Native/Bilingual            & 27.9      & 53.8    \\ \hline
\end{tabular}
\caption{Detection rate based on language proficiency. Superscripts indicate statistical difference observed with Mann Whitney U Test($\alpha=0.01$)}
\label{table:rq3_language}
\end{table}

\textbf{Grammaticality}
Lastly, we study the effect that language proficiency has on our results.  Table \ref{table:rq4_language} shows  the language proficiency does not  have an effect on the errors reported for adversarial examples.  However, it affects the reported rate of errors introduced by adversarial examples on original text. More proficient participants report more added errors, with Native/bilinguals reporting up to 13.3\% more added errors. 

\begin{table}[ht!]
\begin{tabular}{@{}lll@{}}
\toprule
Language proficiency & Errors     & Errors     \\
                     & present    & added      \\ \midrule
Limited working      & 38.8(17.6) & 31.7(12.4) \\
Professional         & 38.3(18)   & 40.1(13.1) \\
Native/bilingual     & 39.7(17.3) & 45.0(11.6)  
\end{tabular}
\caption{Percentage of grammar errors detected by human evaluators  according to their language proficiency. The numbers in brackets represent the errors found automatically with LanguageTools grammar checker. }
\label{table:rq4_language}
\end{table}


\textbf{Meaning}

Finally, we investigate the influence of language proficiency in our results. According to the data in Table \ref{table:rq5_language},  the proficiency level does not statistically affect the clarity of the meaning. Regarding meaning preservation, the group with limited working proficiency assigns a statistically higher score than the native/bilingual group. 

\begin{table}[ht!]
\begin{tabular}{lll}
\hline
Language proficiency              & Meaning & Preservation \\ \hline
$^{a}$Limited working  & 2.65  & 2.26 $^{c}$ \\
$^{b}$Professional     & 2.63  & 2     \\
$^{c}$Native/Bilingual            & 2.55  & 2.15 $^{a}$ \\ \hline
\end{tabular}
\caption{Clarity of the meaning and meaning preservation based on language proficiency. Superscripts indicate statistical difference observed with Mann Whitney U Test($\alpha=0.01$)}
\label{table:rq5_language}
\end{table}

\noindent\fbox{%
    \parbox{\columnwidth}{% 
  Humans find that adversarial text is less meaningful than original text. They as well report that adversarial text somehow preserves the meaning of the original text, but not completely. Higher adversarial perturbation size, renders the text less meaningful and reduces its meaning preserving capabilities. The language proficiency does not have a strong effect on the results reported by humans. 
    }%
}
